Convex Relaxation of Optimal Power Flow, Part I: Formulations and Equivalence

This tutorial summarizes recent advances in the convex relaxation of the optimal power flow (OPF) problem, focusing on structural properties rather than algorithms. Part I presents two power flow models, formulates OPF and their relaxations in each model, and proves equivalence relations among them. Part II presents sufficient conditions under which the convex relaxations are exact.

==> 1-models-v1.tex <==

\section{Power flow models}
\label{sec:models}

In this section we describe two power flow (or load flow) models, prove
their equivalence, and discuss their applications.

\subsection{Bus injection model}

Consider a power network  modeled by a connected undirected graph 
$G(N^+, E)$ where $N^+ := \{0\} \cup N$, $N := \{1, 2, \ldots, n \}$,
and $E \subseteq N^+ \times N^+$.   Each node in $N^+$ represents a bus 
and each edge in $E$ represents a line.  For each edge $(i,j)\in E$
let $y_{ij}$ be its admittance.
A bus $j \in N^+$ can have a generator, a load, both or neither.  
For economic dispatch, the loads are specified and the generations are variables to be determined;
for demand response applications, the loads are optimization variables as well.
Let $V_j$ be the complex voltage at bus $j \in N$ and $|V_j|$ denote its magnitude.
 Bus 0 is the \emph{slack bus}.  Its voltage is fixed and we assume without loss of generality
 that $V_0 = 1\angle 0^\circ$ p.u.
Let $s_j$ be the net complex power injection
(generation minus load) at bus $j\in N^+$.
We use $s_j$ to denote both the complex number $p_j + \ii q_j$ and the real pair $(p_j, q_j)$
depending on  the context.


The \emph{bus injection model} is defined by the following power flow equations
that describe the Kirchhoff's law: 
\bq
s_j  & = & \sum_{k: j\sim k} y_{jk}^H\ V_j (V_j^H - V_k^H),
\ \ \  j \in N^+
\label{eq:bim.1}
\eq

 
The \emph{power flow} or \emph{load flow} problem is: given the slack bus voltage
$V_0$ and power injections $s := (s_1, \dots, s_n)$, solve the $n+1$ equations in
\eqref{eq:bim.1} for the complex variables $(V, s_0) \in \mathbb C^{n+1}$.    This 
represents the case, e.g.,
where buses $j\in N$ are buses with constant-power loads $s$ supplied by the 
generator at the slack bus $0$.
For \emph{optimal} power flow problems $s$ are variables as well.

Define the set of power flow solutions as a function of power injections $s$ by:
\begin{align}
\mathbb{V}(s) := \{ V \in \mathbb{C}^n \ \vert \ V \text{ satisfies } \eqref{eq:bim.1} \}
\label{eq:defVs}
\end{align}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Branch flow model}
\label{sec:bfm}

In the branch flow model we adopt a directed connected graph 
$\tilde G = (N^+, \tilde E)$ to represent a power network where each
node in $N^+ := \{0, 1, \dots, n\}$ represents a bus and each edge in $\tilde E$ represents a line.
Fix an arbitrary orientation for $G$ and let 
 $m := |\tilde E|$ be the number of directed edges in $G$.
%
% We adopt the following orientation for $\tilde G$ for convenience (only).
% Pick {\em any} spanning tree $T := (N, \tilde{E}_T)$ of $G$  rooted at the slack bus 1,
% i.e., $T$ is connected and $\tilde{E}_T \subseteq \tilde{E}$ has $n-1$ edges.  
% All edges in $\tilde{E}_T$ point away from the root.   For any edge in 
% $\tilde E\setminus \tilde{E}_T$ that is not in the spanning tree $T$, pick an arbitrary direction.    
Denote an edge by $(i, j)$ or $i\rightarrow j$ if it points from bus $i$ to bus $j$.    
For each edge $(i,j)\in \tilde E$ let $z_{ij}:= 1/y_{ij}$ be the complex impedance on the line, 
%
 let $I_{ij}$ be the complex current from buses $i$ to $j$, and 
$S_{ij} = P_{ij} + \ii Q_{ij}$ be the {\em sending-end} complex power from buses $i$ to $j$.
For each bus $i\in N^+$ let $V_i$ be the complex voltage at bus $i$.
Let $s_i$ be the net complex power injection (generation minus load) at bus $i$.

The \emph{branch flow model} is defined by the following set of power flow equations:
\begin{subequations}
\bq
\!\!\!\!
% s_j  & \!\! = \!\! &\!\!\!\!  \sum_{k: j\rightarrow k} \!\!\! S_{jk} - \!\!\!
\sum_{k: j\rightarrow k} \!\!\! S_{jk}  & \!\! = \!\! &\!\!\!\!   
	\sum_{i: i\rightarrow j} \!\! \left( S_{ij} - z_{ij} |I_{ij}|^2 \right) + s_j, 	\,  j \in N^+
\label{eq:bfm.3}
\\
\!\!\!\!
I_{jk}  & \!\! = \!\! &  y_{jk} (V_j - V_k),  \quad j \rightarrow k \in \tilde{E}
\label{eq:bfm.1}
\\
\!\!\!\!
S_{jk}  & \!\! = \!\! & V_j \ I_{jk}^H, \quad j \rightarrow k \in \tilde{E}
\label{eq:bfm.2}
\eq
\label{eq:bfm}
\end{subequations}
where \eqref{eq:bfm.1} describes the Ohm's law, \eqref{eq:bfm.2} defines branch power
in terms of the associated voltage and current, and \eqref{eq:bfm.3} imposes 
power balance at each bus.  The quantity
$z_{ij} |I_{ij}|^2$ represents line loss so that $S_{ij} - z_{ij} |I_{ij}|^2$ is the
receiving-end complex power at bus $j$ from bus $i$.

Given $V_0$ and $s$ define the set of solutions $\tilde{x} := (S, I, V, s_0)$
of the branch flow model by:
\begin{align}
\mathbb{\tilde{X}}(s) := \{ \tilde{x} \in \mathbb{C}^{2m+n+1} \ \vert \ \tilde{x} \text{ satisfies } 
				\eqref{eq:bfm} \}
\label{eq:defXs}
\end{align}


\subsection{Equivalence}

Even though the bus injection model and the branch flow model are defined by different
sets of equations in terms of their own variables, both are models of the Kirchhoff law
and therefore must be related.  We now clarify the precise sense in which these two
mathematical models are equivalent.  
We say two sets $A$ and $B$ are \emph{equivalent}, denoted $A\equiv B$, if
there is a bijection between them.
\begin{theorem}
\label{thm:bim=bfm}
$\mathbb V(s) \equiv \mathbb{\tilde X} (s)$ for any power injections $s$.
\end{theorem}

\begin{proof}
Fix any injections $s\in \mathbb C^n$.
It suffices to show that there is a bijection between the set of $V$ that satisfy
\eqref{eq:bim.1} and the set of $(S, I, \tilde V, s_0)$ that satisfy \eqref{eq:bfm}.
Here we use $V$ to denote a power flow solution in $\mathbb V$ and $\tilde V$ to 
denote a component of a power flow solution in $\mathbb X$.
We now exhibit a function $g$ that maps $V$ to $(S, I, \tilde V, s_0)$
and its inverse $g^{-1}$.

To construct $g$, fix any $V$ that satisfies \eqref{eq:bim.1}.
Define $s_0(V)$ by \eqref{eq:bim.1}, $\tilde V := V$, $I(V)$ by \eqref{eq:bfm.1}.  
Then define $S_{jk}(V)$ by \eqref{eq:bfm.2} (only) for $j\rightarrow k \in \tilde E$.  
This specifies $g(V) := (S(V), I(V), \tilde V(V), s_0(V))$.     We only need to show that
$g(V)$ satisfies \eqref{eq:bfm.3}.  For each $i\rightarrow j \in \tilde E$ we have
by construction (recall $y_{jk} = y_{kj}$)
\bqn
S_{ij}(V) - z_{ij} |I_{ij}(V)|^2 & = & 
y_{ij}^H\ V_i (V_i - V_j)^H - y_{ij}^H\ |V_i - V_j|^2
\\
& = & - y_{ij}^H\ V_j (V_j - V_i)^H
\eqn
Hence for each $j\in N^+$
\bqn
& & \sum_{k: j\rightarrow k} S_{jk}(V)  \, -   
	\sum_{i: i\rightarrow j}  \left( S_{ij}(V) - z_{ij} |I_{ij}(V)|^2 \right)
\\
& = & \sum_{k: j\rightarrow k} y_{jk}^H\ V_j (V_j - V_k)^H \, + 
	\sum_{i: i\rightarrow j}  y_{ij}^H\ V_j (V_j - V_i)^H
\\
& = & \sum_{k: j\sim k} y_{jk}^H\ V_j (V_j^H - V_k^H) \ = \ s_j(V)
\eqn
which is \eqref{eq:bfm.3}.

Conversely, given an $(S, I, \tilde V, s_0)$ that satisfies \eqref{eq:bfm}, 
define $V := g^{-1}(S, I, \tilde V, s_0) := \tilde V$.  
That $(S, I, \tilde V, s_0)$ satisfies \eqref{eq:bfm} implies that $g^{-1}$
as defined is indeed the inverse of $g$ above.  Moreover 
\eqref{eq:bfm.3} implies that $V$ satisfies \eqref{eq:bim.1}.
\end{proof}
\vspace{0.1in}

Given the bijection between the solution sets $\mathbb V(s)$ and $\mathbb{\tilde X}(s)$
any result in one model is in principle derivable in the other model.   
As we will see later however
some results are much easier to state or derive in one model than the other.  
For instance semidefinite relaxation of power flows has a much cleaner formulation
in the bus injection model.  
The branch flow model, especially for radial networks, has a convenient 
recursive structure that allows a more efficient computation of power flows; 
moreover the derivation of some of the sufficient conditions for exact relaxation 
rely critically on this recursive structure; see Section \ref{subsec:bfmr}.
 Since the variables in
the branch flow model correspond directly to physical quantities such as
branch power flows and injections it is sometimes more convenient in
applications.    
 We will therefore freely use either model depending on
which is more convenient for the problem at hand.  


\begin{comment}
\subsection{Linear approximations}
\label{subsec:la}

\noindent
\textbf{DC power flow in bus injection model.}
A popular linear approximation of the bus injection model is called the \emph{DC power flow}
or \emph{DC approximation} \cite{Stott1974,Alsac1990,Purchala2005,Stott2009}.
It makes the following assumptions:
\bee
\item[1.] Voltage magnitudes are fixed at $|V_j| = 1$ pu.
\item[2.] The angle differences $|\theta_j -\theta_k|$ on the voltages are small across each line $(i,j)$
	so that $(\theta_j - \theta_k)^2$ is negligible.
\eee
Assumption 1 means that the voltage variables $V_j = e^{\ii \theta_j}$
reduce to their phase angles $ \theta_j$.   Assumptions 2 then justifies
the following first-order Taylor approximation 
\bqn
V_j( V_j - V_k )^H & = & 1 - e^{\ii (\theta_j - \theta_k)} \ \simeq \ - \ii (\theta_j - \theta_k)
\eqn
Substituting into \eqref{eq:bim.1} we have
\bqn
s_j & = & \sum_{k: j\sim k} -\ii \, y_{jk}^H\ (\theta_j - \theta_k), \quad j \in N^+
\eqn
This can be expressed in vector form by treating the graph as directed as in 
$\tilde G = (N^+, \tilde E)$ with an arbitrary orientation.   Define the $(n+1) \times m$ incidence 
matrix $C$ with
\bqn
C_{jl} & = & \left\{\begin{array}{rcl}
	1 & & \text{ if } l = (j, k) \in \tilde E
	\\
	-1 & & \text{ if } l = (i, j) \in \tilde E
	\\
	0  & & \text{ otherwise}
	\end{array} \right.
\eqn
Then linear approximation of \eqref{eq:bim.1} becomes
\bq
\tilde s & = & C \, \text{diag} \left( -\ii \, y_{jk}^H \right) \, C^T \theta
\label{eq:DCs}
\eq
where $\tilde s := (s_0, s)$.
Standard DC approximation makes the further assumption:
\bee
\item[3.] The lines are lossless so that $z_{jk} = \ii x_{jk}$ and $y_{jk} = -\ii / x_{jk}$.
\eee
The linear approximation \eqref{eq:DCs} then involves only real power:
\\
\noindent
\textbf{DC approximation:}
\bq
\tilde p & = & C \, \text{diag} \left( x_{jk}^{-1} \right) \, C^T \theta
\label{eq:DCp}
\eq
where $\tilde p := \text{Re}\, \tilde s$.
This is the most common form of DC approximation of the bus injection model
and widely used in practice, e.g., in electricity market operation.
The matrix $C \, \text{diag} \left( x_{jk}^{-1} \right) \, C^T$ is $(n+1) \times (n+1)$
but has rank $n$.  Since we fix $\theta_0$ to be 0 (without loss of generality) at the slack bus 
\eqref{eq:DCp} uniquely determines a $\theta$ given a real power injection $p$.

\vspace{0.1in}
\noindent
\textbf{Linear approximation in branch flow model.}
We can derive a linear approximation of the branch flow model 
\eqref{eq:bfm} as follows.   
First combine \eqref{eq:bfm.1}--\eqref{eq:bfm.2} into:
\bqn
V_k & = & V_j \ - \ z_{jk}\, \frac{S_{jk}^H}{V_j^H}
\eqn
and take the magnitude square:
\bq
v_k & = & v_j - 2\, \text{Re} \ z_{jk}^H \, S_{jk} + |z_{jk}|^2 |I_{jk}|^2
\label{eq:linv}
\eq
where $v_j := |V_j|^2$.
Omitting the quadratic term yields a linear equation in $(S, v)$:
\bqn
v_j - v_k & = & 2 (r_{jk} P_{jk} + x_{jk} Q_{jk}), \quad j\rightarrow k \in \tilde E
\eqn
where $z_{jk} =: (r_{jk}, x_{jk})$ and $S_{jk} =: (P_{jk}, Q_{jk})$.\footnote{We abuse notation
and use $z$ and $S$ both to denote complex variables in $\mathbb C^{m}$ and as a
shorthand for the real variables $(r, x)$ and $(P, Q)$ in $\mathbb R^{2m}$.}
Then omitting the line losses $z_{jk}|I_{jk}|^2$ in \eqref{eq:bfm.3} yields
\bqn
s_j & = & \sum_{k: j\rightarrow k} \!\!\! S_{jk} - \sum_{i: i\rightarrow j} \!\!  S_{ij},	\quad j \in N^+
\eqn
To write this in vector form let diag$(z_{jk}^T)$ be the $m \times 2m$ block diagonal matrix
where the $(j,k)$th row consists of the 2-dimensional row vector $[r_{jk}\  \, x_{jk}]$.   
We abuse notation and use $S$ to also denote a $2m$-dimensional vector in $\mathbb R^{2m}$
consisting of $[P_{jk}\ \, Q_{jk}]^T$, $j\rightarrow k\in \tilde E$, stacked together.
Then the linear
approximation of the branch flow model \eqref{eq:bfm} in terms of the
variables $(S, v, s_0) =: (S, v, \tilde s) \in \mathbb R^{2m + n + 1}$ is:
\bq
\tilde s & = & C\, S
\label{eq:linbfm.1}
\\
C^T\, v & = & 2\ \text{diag} \left( z_{jk}^T \right) S
\label{eq:linbfm.2}
\eq
% \bqn
% s_j & = & \sum_{k: j\rightarrow k} \!\!\! S_{jk}   - 
% 	\sum_{i: i\rightarrow j} \!\!  S_{ij}, 	\quad j \in N^+
% \\
% v_k & = & v_j - 2\, \text{Re} z_{jk}^H S_{jk} 
% \eqn
\end{comment}

\subsection{BFM for radial networks}
\label{subsec:bfmr}

Branch flow models have mainly been used for distribution systems where
networks are usually radial (having a tree topology), e.g.
\cite{Baran1989a, Baran1989b, ChiangBaran1990, Chiang1991,
Cespedes1990, Exposito1999, Jabr2006, Farivar2011-VAR-SGC, Taylor2012-TPS}.
These models take a recursive form for radial networks.
The recursive structure is an important advantage that simplifies the 
computation of power flow solutions
e.g. \cite{Kersting2002, Shirmohammadi1988, ChiangBaran1990}.   It
is also critical in deriving certain sufficient conditions
for exact relaxation as we will see in Part II of the paper.

We now explain how the model first proposed in
\cite{Baran1989a, Baran1989b} for distribution networks can be derived
as a relaxation of our branch flow model \eqref{eq:bfm}.    We then present
simple bounds on branch power flows and voltage magnitudes based on
linear approximation of the branch flow model for radial networks. 


\subsubsection{Recursive equations}
\label{subsubsec:re}

A key feature in the model of \cite{Baran1989a, Baran1989b} is the absence
of voltage phase angles.   
% The derivation of \eqref{eq:linv} from  \eqref{eq:bfm.1}--\eqref{eq:bfm.2}
% eliminates the phase angles from the complex voltages $V$ and 
Use  \eqref{eq:bfm.1}--\eqref{eq:bfm.2} to eliminates the phase angles from 
the complex voltages $V$ and currents $I$, and 
taking the magnitude square of \eqref{eq:bfm.2} we 
arrive at the following set of recursive equations for a radial network
\cite{Farivar-2013-BFM-TPS}:
\begin{subequations}
\bq
\sum_{k: j\rightarrow k} S_{jk} & = & S_{ij} - z_{ij} \ell_{ij} + s_j, \quad j \in N
\label{eq:df.1}
\\
v_j - v_k & = & 2\, \text{Re} \left(z_{jk}^H S_{jk} \right) - |z_{jk}|^2 \ell_{jk}, \ \ j\rightarrow k \in \tilde E
\nonumber
\\
\label{eq:df.2}
\\
\ell_{jk} v_j & = & |S_{jk}|^2, \quad j\rightarrow k \in \tilde E
\label{eq:df.3}
\eq
\label{eq:df.a}
\end{subequations}
where bus $i$ in \eqref{eq:df.1} denotes the unique parent of bus $j$
(on the unique path from bus 0 to bus $j$).
Without loss of generality bus 0 is taken as the root of the tree.  For distribution
systems it usually represents a substation bus.
Suppose we adopt a graph orientation where every link points away from
the root of the tree (bus 0).   Then the boundary conditions  
for \eqref{eq:df.1} when $j = 0$ or when $j$ is a leaf node are:
\begin{subequations}
\bq
s_0 & = & \sum_{k: 0\rightarrow k} S_{0k} 
\label{eq:df.4}
\\
s_j & = & - S_{ij} + z_{ij} \ell_{ij}   \ \ \text{ if $j$ is a leaf node}
\label{eq:df.5}
\eq
\label{eq:df.b}
\end{subequations}
The model \eqref{eq:df.a}--\eqref{eq:df.b} is called the \emph{DistFlow} equations
and first proposed in \cite{Baran1989a, Baran1989b}.

This transformation defines a mapping   
$h : \mathbb C^{2m+n+1} \rightarrow \mathbb R^{3m+n+2}$ that maps
a power flow solution $\tilde x = (S, I, V, s_0)$ to $h(\tilde x) = x := (S, \ell, v, s_0)$ with 
$\ell_{jk} = |I_{jk}|^2$ and $v_j = |V_j|^2$.
Given power injections $s \in \mathbb R^{2n}$ define the set of solutions 
$x := (S, \ell, v, s_0)$ of the DistFlow equations as:
\bqn
{\mathbb X}_{r}(s) & := & \{ x \in \mathbb R^{3m+n+2} \ \vert \ x \text{ satisfies } 
		\eqref{eq:df.a}-\eqref{eq:df.b} \}
\eqn
The model \eqref{eq:df.a} is a relaxation of the branch flow model \eqref{eq:bfm}
in the sense that, for any $\tilde x \in \mathbb{\tilde X}(s)$, $h(\tilde x) \in \mathbb X_r(s)$.
For radial networks it turns out that the converse is true, i.e., there is a bijection
between $\mathbb{\tilde X}(s)$ and $\mathbb X_r(s)$; see Theorem \ref{thm:bfm.1}
in Section \ref{subsec:Relabfm}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\subsubsection{Solution methods}

\slow{Remove this sub-subsection for TCNS submission.}
One way to understand the structure of the power flow problem is given in 
\cite{ChiangBaran1990}.  
Suppose without loss of generality that the network graph is oriented so that every
link in the graph points away front the root of the tree (bus 0).
Consider first the special case of a linear network that represents the main feeder
shown in Figure \ref{fig:mainfeeder}.
\slow{Add figure with two subfigures: (a) Main feeder.  (b) Main feeder with laterals.}
To simplify notation denote $\left(S_{j(j+1)}, \ell_{j(j+1)} \right)$ and $z_{j(j+1)}$ by 
$(S_j, \ell_j)$ and $z_j$ respectively.  Then the DistFlow equations 
\eqref{eq:df.a}--\eqref{eq:df.b} reduce to:
\begin{subequations}
\bq
S_{j+1} & = & S_{j} - z_{j} \ell_{j} + s_{j}, \ \  j = 0, \dots, n-1
\label{eq:cb.1}
\\
v_{j+1}& = & v_j - 2 \text{Re} (z_{j}^H S_{j}) - |z_{j}|^2 \ell_{j}, \ \ j = 0, \dots, n-1
\nonumber
\\
\label{eq:cb.2}
\\
\ell_{j} v_j & = & |S_{j}|^2, \ \  j = 0, \dots, n-1
\label{eq:cb.3}
\\
S_n & = & 0
\label{eq:cb.4}
\\
v_0 & \text{ is } & \text{given}
\nonumber
\eq
\end{subequations}
We have omitted $s_0$ as a variable with the understanding that $s_0 = S_0$.
Let $w_j := (S_j, \ell_j, v_j)$, $j = 0, \dots, n$.  If $S_0$ is known then
one can start with $(v_0, S_0)$ and use the recursion \eqref{eq:cb.1}--\eqref{eq:cb.3} 
to compute $w_j$ in terms of $S_0$, i.e., \eqref{eq:cb.1}--\eqref{eq:cb.3} can
be collapsed into simple functions of the scalar variable $S_0$:
\bq
w_j & = & f_j(S_0), \quad j=0, \dots, n
\label{eq:lnDF.sol1}
\eq
Use the boundary condition \eqref{eq:cb.4}
\bq
S_n & = & f_{n1}(S_0) \ = \ 0
\label{eq:lnDFsol2}
\eq
to solve for the scalar variable $S_0$.   The other variables $w_j$ can then be easily computed
from \eqref{eq:lnDF.sol1}.

This method can be extended to a general radial network with laterals.  
Call bus $k$ a \emph{junction bus} if there are laterals or sublaterals branching off 
from bus $k$; see Figure \ref{fig:laterals}.   If there are $n_k$ branches going out from
bus $k$ (in the direction pointing away from bus $0$) then we say bus $k$ has an 
\emph{out-degree} of $n_k$.  
\slow{Caption in the Figure give examples of ``out-degree'' of a junction bus.}  
Let  the total number of branches going out from all junction buses be denoted by
\bqn
K  & := &  \sum_{\text{junction buses $k$}} n_k
\eqn
Let $\tilde S \in \mathbb C^K$ be the vector of branch power flows
on these branches.  
Then the extension of the above method from a general radial  network to a tree modifies the single
nonlinear equation \eqref{eq:lnDFsol2} in the scalar variable $S_0$
to $K$ nonlinear equations in the $K$ dimensional vector variable $\tilde S$, of the form:
\bq
f(\tilde S) & = & 0
\label{eq:DFsol}
\eq
\slow{Provide example using Figure \ref{fig:laterals}?}
Even though \eqref{eq:DFsol} may have multiple solutions it is argued in \cite{ChiangBaran1990}
that, under appropriate conditions, only a single solution is practical in that all other solutions
have voltage magnitudes close to 0 pu instead of 1 pu.
Solving the nonlinear equations \eqref{eq:DFsol} can in general be difficult and
various techniques have been developed to reduce the computational complexity;
see e.g. \cite{ZimmermanChiang1995, Srinivas2000} and references therein.

A different approach called the \emph{forward/backward sweep} makes use of the
recursive structure of \eqref{eq:df.a} to compute a solution iteratively
\cite{Kersting2002, Shirmohammadi1988}.  
\slow{See other references in \cite{ZimmermanChiang1995}.}
The algorithm in \cite{Shirmohammadi1988} proceeds as follows:
\slow{This uses complex formulation of full branch flow model, not DistFlow 
equations?}
\bee
\item \emph{Compute current injections.} Given the voltages 
	$V^t := (V_1^t, \dots, V_n^t)$ in the $t$-th
	iteration, compute the current injections at every bus using 
	$i_j^t := (s_j / V_j^t)^H$.
\item \emph{Backward sweep.} Starting from the leaf nodes and working towards the 
	root, compute branch currents $- I_{ij}^t := i_j^t - \sum_{k: j\rightarrow k} I_{jk}^t$
	using the KCL, where $i\rightarrow j$ is the link on the unique path from the root
	(bus $0$) to bus $j$ and $j\rightarrow k$ are links from bus $j$ to bus $k$ in
	the direction pointing away from the root.
\item \emph{Forward sweep.}  Starting front the root (with given $V_0$) and working 
	towards the leaf nodes, compute the nodal voltages $V_j^{t+1} := V_i^{t+1} - Z_{ij}I_{ij}^t$
	using the KVL and the branch currents $I_{ij}^t$ computed from the backward sweep.	
\eee
The initial voltages can be set to $1\angle 0^\circ$ pu (except for $V_0$ which is given).
These iterations are then repeated until convergence. 

\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsubsection{Graph orientation}

The model \eqref{eq:df.a} is defined for any graph orientation.    Different
orientations may have different boundary conditions \eqref{eq:df.b}.
It is customary in the literature to orient the graph so that every link
points away from the root of the tree (bus 0) as this simplifies the presentation or 
derivation of certain results (e.g., Theorem 2 in \cite{Farivar-2013-BFM-TPS1}).
Sometimes it is more convenient to use the opposite orientation where every link 
points towards bus 0; see Section \ref{subsubsec:sb} below.

Indeed the variables for these two opposite orientations have a familiar relation 
as we now explain.  
Suppose the network is oriented so that all links point away from bus 0 and the corresponding
recursive equations are \eqref{eq:df.a} with the boundary conditions \eqref{eq:df.b}.   
Fix this orientation and define the following functions:
\bqn
\hat{S}_{kj} :=\, \hat{S}_{kj}(S, \ell, v) & := & - (S_{jk} - z_{kj} {\ell}_{kj}),  \  j\rightarrow k \in E
\\
\hat{\ell}_{kj} :=\,  \hat{\ell}_{kj}(S, \ell, v) & := & \ell_{jk},  \quad  j\rightarrow k \in E
\\
\hat v_j := \, \hat{v}_j(S, \ell, v) & := & v_j, \quad j \in N
\eqn
Note that for each directed link $j\rightarrow k \in E$, the branch flow model defines only the variables 
$S_{jk}$ and $\ell_{jk}$, so the above expressions are not relations among the variables
$(S, \ell, v)$ and $(\hat S, \hat \ell, \hat v)$, but  definitions that define
$(\hat S, \hat \ell, \hat v)$ as functions of $(S, \ell, v)$.
Since $S_{jk}$ represents the sending-end complex power from bus $j$ to bus $k$, 
$- \hat S_{kj}(S, \ell, v)$ represents the received power by bus $k$ from bus $j$, net of 
the line loss $z_{jk}\ell_{jk}$.
Substituting these definitions into \eqref{eq:df.a}--\eqref{eq:df.b} yields
\begin{subequations}
\bq
\hat{S}_{ji} - s_j & = & \sum_{k: j\rightarrow k} \left( \hat{S}_{kj} - z_{kj} \hat \ell_{kj} \right)
% , \quad j \in N
\label{eq:bdf.1}
\\
\hat v_k - \hat v_j & = & 2\, \text{Re} \left(z_{kj}^H \hat S_{kj} \right) - |z_{kj}|^2 \hat\ell_{kj}
% , \ \ (j,k) \in E
% \nonumber \\
\label{eq:bdf.2}
\\
\hat\ell_{kj} \hat v_j & = & |\hat S_{kj}|^2
% , \quad (j,k) \in E
\label{eq:bdf.3}
\\
- s_0 & = & \sum_{k: 0\rightarrow k} \left( S_{k0} - z_{k0} |\hat I_{k0}|^2 \right)
\label{eq:bdf.4}
\\
s_j & = & \hat{S}_{ji}  \ \ \text{ if $j$ is a leaf node}
\label{eq:bdf.5}
\eq
\label{eq:bdf}
\end{subequations}
where as before $i$ in \eqref{eq:bdf.1} and \eqref{eq:bdf.5}
is the unique parent of node $j$ (i.e., the node on the unique path between 
node 0 and node $j$).  Here \eqref{eq:bdf.3} follows from \eqref{eq:df.3} because:
\bqn
\hat\ell_{kj} \hat v_j & = & \left| \hat S_{kj} - z_{kj}\hat\ell_{kj} \right|^2
\\
& = & \left| \hat S_{kj} \right|^2 +  \left( \left| z_{kj} \right|^2 \hat\ell_{kj} - 
			2\, \text{Re} \left( z_{kj}^H \hat S_{kj} \right) \right) \hat\ell_{kj}
\eqn
This together with \eqref{eq:bdf.2} imply \eqref{eq:bdf.3}.

As mentioned above the expressions $(\hat S, \hat \ell, \hat v)$
 in \eqref{eq:bdf} are functions of the variables
$(S,\ell, v)$ defined for a given graph orientation.
If however we reverse the direction of all the links  then \eqref{eq:bdf} become exactly the
recursive equations for the network with the opposite orientation, 
where $(\hat S, \hat \ell, \hat v)$ are not functions but themselves variables that 
define the model.    We therefore can
either think of \eqref{eq:bdf} as defining a branch flow model in terms of $(\hat S, \hat \ell, \hat v)$
with a new graph orientation, 
or as some properties of the original model \eqref{eq:df.a}--\eqref{eq:df.b},
expressed in terms of the functions $(\hat S, \hat \ell, \hat v)$, that are satisfied by the variables
$(S, \ell, v)$. 
These are equivalent models (with different boundary conditions)
and we will freely use whichever one is more convenient for the question under study.\footnote{An alternative model
is to use an undirected graph and, for each link $(j,k)$, both the variables $S_{jk}$ and $S_{kj}$ are
defined with the additional equations $S_{jk} + S_{kj} = z_{jk}\ell_{kj}$.
}

The orientation where all links point towards bus 0  sometimes has an advantage in 
power flow calculation
because, when $s$ (but not $s_0$) is given, \eqref{eq:bdf.4} provides an easy 
initiation of the recursion.
This leads to an easy derivation of upper bounds on $v_j$ as explained in
Lemma \ref{lemma:ldf2} below.
% Another more subtle advantage is illustrated in Section \ref{gan}.


\subsubsection{Simple bounds}
\label{subsubsec:sb}

% A linearized model in Section \ref{subsec:la} takes the following form for radial networks
By setting $\ell_{jk}=0$ in  \eqref{eq:df.a}--\eqref{eq:df.b}
we obtain a linear approximation of the the branch flow model
(assuming the graph orientation where all links point away from bus $0$):
\begin{subequations}
\bq
\sum_{k: j\rightarrow k} S^{\text{lin}}_{jk} & = & S^{\text{lin}}_{ij}  + s_j, \quad j \in N
\label{eq:ldf.1}
\\
v^{\text{lin}}_j - v^{\text{lin}}_k & = & 2\, \text{Re} \left(z_{jk}^H S^{\text{lin}}_{jk} \right), \ \ (j,k) \in E
\label{eq:ldf.2}
\\
s_0 & = & \sum_{k: 0\rightarrow k} S_{0k}^{\text{lin}} 
\label{eq:ldf.3}
\\
s_j & = & - S_{ij}
\label{eq:ldf.4}
\eq
\label{eq:ldf}
\end{subequations}
where bus $i$ in \eqref{eq:ldf.1} and \eqref{eq:ldf.4} denotes the unique parent of bus 
$j$.   This is called the \emph{simplified DistFlow equations} in \cite{Baran1989b, Baran1989c}.
It is a reasonable approximation of \eqref{eq:df.a} because the loss $z_{jk}\ell_{jk}$
is typically much smaller than the branch power flow $S_{jk}$.

The following result provides simple bounds on the branch flow variables $(S, v)$ in
terms of their linear approximations $(S^{\text{lin}}, v^{\text{lin}})$ and are useful in 
proving several results on exact relaxation.
 They can be easily derived using the recursive structure of \eqref{eq:df.a} and
 their linear approximation \eqref{eq:ldf}.
 Denote by $\mathbb T_j$ the subtree rooted at bus $j$, including $j$.
We write ``$k\in \mathbb T_j$'' to mean node $k$ of $\mathbb T_j$ and
``$(k, l)\in \mathbb T_j$'' to mean edge $(k,l)$ in $\mathbb T_j$.
Denote by $\mathbb P_k$ the set of links on the unique path from bus 0 to bus $k$.

\begin{lemma}
\label{lemma:ldf1} Fix any $v_0$ and $s$.
Let $x := (S, \ell, v, s_0)$  and
$x^{\text{lin}} := (S^{\text{lin}}, \ell^{\text{lin}}, v^{\text{lin}}, s_0^{\text{lin}})$ be solutions
of \eqref{eq:df.a}--\eqref{eq:df.b} and \eqref{eq:ldf} respectively. 
Then
\bee
\item[(1)] For $(i,j)\in E$
	\bqn
	S^{\text{lin}}_{ij} & = & - \sum_{k \in \mathbb T_j} s_k
	\\
	S_{ij} & = & - \sum_{k\in \mathbb T_j} s_k\ + \left( z_{ij} \ell_{ij} + \sum_{(k,l)\in \mathbb T_j} z_{kl} \ell_{kl} \right)
	\eqn
\item[(2)] For $(i,j)\in E$, $S_{ij} \geq S^{\text{lin}}_{ij}$ with equality only if all $\ell_{kl}$ 
	 in $\mathbb T_j$ are zero.

\item [(3)]For $j\in N^+$
	\bqn
	v^{\text{lin}}_{j} & = & v_0 \ - 
			 \sum_{(i,k) \in \mathbb P_j} 2\, \text{Re} \left( z_{ik}^H S_{ik}^{\text{lin}} \right)
	\\
	v_{j} & = & v_0 \ -  \sum_{(i,k) \in \mathbb P_j} \left( 2\, \text{Re} \left( z_{ik}^H S_{ik} \right) -
					|z_{ik}|^2 \ell_{ik} \right)
	\eqn
\item[(4)] For $j\in N^+$, $v_j \leq  v_j^{\text{lin}}$.
\eee
\end{lemma}

Lemma \ref{lemma:ldf1} says that the power flow $S_{ij}$ on line $(i,j)$ equals the total load 
$- \sum_{k \in \mathbb T_j} s_k$ in the subtree rooted at node $j$ plus the total line loss
in supplying these loads.  
The linear approximation $S_{ij}^{\text{lin}}$ neglects the line losses and underestimates 
the required power to supply these loads.

Lemma \ref{lemma:ldf1}(1)--(3) can be easily proved by recursing on 
\eqref{eq:df.1}--\eqref{eq:df.2} and \eqref{eq:ldf.1}--\eqref{eq:ldf.2}.
The easiest way to prove Lemma \ref{lemma:ldf1}(4) is to make use of the properties 
in \eqref{eq:bdf} as we now explain
(recall that $v_j = \tilde v_j$ and $v_j^{\text{lin}} = \tilde v_j^{\text{lin}}$).

In fact we will think of \eqref{eq:bdf} as the branch flow model for the graph orientation 
where all links point towards bus 0.   Then the linearized model corresponding to 
\eqref{eq:bdf} is (setting $\ell_{kj}=0$):
\begin{subequations}
\bq
\hat{S}_{ji}^{\text{lin}} & = & \sum_{k: k\rightarrow j}  \hat{S}_{kj}^{\text{lin}}  + s_j, \quad j \in N
\label{eq:lbdf.1}
\\
\hat v_k^{\text{lin}}  - \hat v_j^{\text{lin}}  & = & 
		2\, \text{Re}\! \left(z_{kj}^H \hat S_{kj}^{\text{lin}}  \right)\!, \  (k, j) \in E
\label{eq:lbdf.2}
\\
s_0 & = & - \sum_{k: k\rightarrow 0} \hat{S}_{k0}^{\text{lin}}
\label{eq:lbdf.4}
\\
s_j & = & \hat{S}_{ji}^{\text{lin}}   \ \text{ if $j$ is a leaf node}
\label{eq:lbdf.5}
\eq
\label{eq:lbdf}
\end{subequations}

\begin{lemma}
\label{lemma:ldf2} Fix any  $v_0$ and $s$. 
Let $\hat x := (\hat S, \hat \ell, \hat v, \hat s_0)$ and
$\hat x^{\text{lin}} := (\hat S^{\text{lin}}, \hat\ell^{\text{lin}}, \hat v^{\text{lin}}, \hat s_0^{\text{lin}})$ 
be solutions of \eqref{eq:bdf} and \eqref{eq:lbdf} respectively. 
Then
\bee
\item[(1)] For all $j\rightarrow i \in E$
	\bqn
	\hat S^{\text{lin}}_{ji} & = & \sum_{k \in \mathbb T_j} s_k
	\\
	\hat S_{ji} & = &  \sum_{k\in \mathbb T_j} s_k\  - \sum_{(k,l)\in \mathbb T_j} z_{kl} \hat \ell_{kl} 
	\eqn
\item[(2)] For all $j \rightarrow i \in E$, $\hat S_{ji} \leq \hat S^{\text{lin}}_{ji}$ with equality only if all $\ell_{kl}$ 
	 in $\mathbb T_j$ are zero.
	 
\item[(3)] For $j\in N^+$
	\bqn
	\hat v^{\text{lin}}_{j} & = & v_0 \ +  \sum_{(i,k) \in \mathbb P_j} 
					2 \, \text{Re} \left( z_{ik}^H \hat S_{ik}^{\text{lin}} \right)
	\\
	\hat v_{j} & = & v_0 \ +  \sum_{(i,k) \in \mathbb P_j} \left( 2 \, \text{Re} \left( z_{ik}^H \hat S_{ik} \right)  
					- |z_{ik}|^2 \hat \ell_{ik} \right)
	\eqn

\item[(4)] For $j\in N^+$, $\hat v_j \leq \hat v_j^{\text{lin}}$.
\eee
\end{lemma}

Lemma \ref{lemma:ldf2} says that the branch power $\hat S_{ji}$ (towards bus 0) equals  the total
power injection $\sum_{k \in \mathbb T_j} s_k$ in the subtree rooted at bus $j$ minus the line losses 
in that subtree.  The linear approximation $\hat S_{ji}^{\text{lin}}$ neglects the line losses and hence
overestimates the branch power flow.
Lemma \ref{lemma:ldf2}(4) follows from Lemma \ref{lemma:ldf2}(2) and (3).
Since $v_j = \hat v_j$ and $v_j^{\text{lin}} = \hat v_j^{\text{lin}}$ it also implies
Lemma \ref{lemma:ldf1}(4).


Finally we note that Lemmas \ref{lemma:ldf1} and \ref{lemma:ldf2} do not depend on 
the quadratic equalities \eqref{eq:df.3} and \eqref{eq:bdf.3} as long as $\ell_{jk}\geq 0$.
In particular the lemmas hold if the equalities have been relaxed to inequalities:
\bqn
\ell_{jk} v_j & \geq & |S_{jk}|^2
\eqn
This will be useful when we later consider the SOCP relaxation of OPF.




==> 1-opf-v1.tex <==

\section{OPF and convex relaxations}
\label{sec:opf}

In this section we  formulate optimal power flow problems, 
derive their convex relaxations, and clarify the relations among these
convex relaxations.   As we will see the key to the design of convex
relaxations is to design convex supersets of the nonconvex feasible
sets of the OPF.

\begin{comment}
\slow{$V$ here mostly means $(V_0, V)$ in $\mathbb C^{n+1}$....
inconsistencies....  $N$ vs $N^+$...}
\end{comment}

\subsection{Optimal power flow}

\subsubsection{Bus injection model}

As mentioned earlier the power flow problem aims to solve the bus injection
model \eqref{eq:bim.1} for $V$ given power injections $s$.   For optimal power
flow $s$ is an optimization variable as well.   In addition to the constraints \eqref{eq:bim.1}
all voltage magnitudes must also satisfy:
 \bq
\underline{v}_j \ \leq &\!\!  |V_j|^2 \! \!&  \leq\  \overline{v}_j, \ \ 
  		j \in N
  \label{eq:opfv}
\eq
\noindent
where $\underline{v}_j$ and $\overline{v}_j$ are given lower and upper bounds on voltages. 
The power injections  are also constrained:
\bq
 \underline{s}_j  \leq s_j \leq \overline{s}_j, \ \ \  j \in N^+
 \label{eq:opfs}
\eq
where $\underline{s}_j$ and $\overline{s}_j$ are given bounds on the net generation
at buses $j$.  
If there is no bound on the load or on the generation at bus $j$
then $\underline{s}_j = -\infty - \ii \infty$ or $\overline{s}_j = \infty + \ii \infty$ respectively.
This is usually the case for $s_0$ at the slack bus 0.
On the other hand this also allows the case where $s_j$ is fixed, e.g., at a constant-power
load bus, by setting $s_j = \underline s_j = \overline{s}_j$ to the specified value.
We can eliminate the variables $s_k$ from the OPF formulation by combining
\eqref{eq:bim.1} and \eqref{eq:opfs} into
\bq
\underline{s}_j  \ \ \leq  \sum_{k: (j, k) \in E} V_j (V_j^H - V_k^H) y_{jk}^H \ \ 
\leq \ \ \overline{s}_j, 
\  j \in N^+
\label{eq:bimopf.1}
\eq
Then OPF in the bus injection model can be defined just in terms of the complex voltage
vector $V$.    Define
\begin{align}
\mathbb{V} := \{ V \in \mathbb{C}^n \ \vert \ V \text{ satisfies } \eqref{eq:opfv}, \eqref{eq:bimopf.1} \}
\label{eq:defV}
\end{align}
$\mathbb V$ is the feasible set of  optimal power flow problems in the bus
injection model.


Let the cost function be $C(V)$.  Typical costs include the cost of
generating real power at each generator bus or line loss over the network.
All these costs can be expressed as  functions of $V$.   Then the problem of interest is:
\\
\noindent
\textbf{OPF:}
\bq
\label{eq:OPFbim}
\underset{V}{\text{min}}   \ C(V) \ & \text{subject to} &   V \in \mathbb V
\eq
Since \eqref{eq:bimopf.1} is quadratic, $\mathbb{V}$ is generally a nonconvex set.
OPF is thus a nonconvex problem and NP-hard to solve in general. 


\subsubsection{Branch flow model}

Denote the variables in the branch flow model \eqref{eq:bfm} by 
$\tilde{x} := (S, I, V, s_0, s) \in \mathbb{C}^{2m+2n+1}$.  
We can also eliminate the variables $s_j$ as for the bus injection model 
by combining \eqref{eq:bfm.3} and \eqref{eq:opfs} 
but it will prove convenient to retain $s_0$ and $s:= (s_j, j\in N)$ as part of the variables.
Define the feasible set in the branch flow model:
\begin{align}
\mathbb{\tilde X} := \{ \tilde{x} \in \mathbb{C}^{2m+2n+1} \ \vert \ \tilde{x} \text{ satisfies } 
				\eqref{eq:bfm},  \eqref{eq:opfv}, \eqref{eq:opfs} \}
\label{eq:deftX}
\end{align}


Let the cost function in the branch flow model be $C(\tilde x)$.
Then the optimal power flow problem in the branch flow model is:
\\
\noindent
\textbf{OPF:}
\bq
\label{eq:OPFbfm}
\underset{\tilde x } {\text{min}}   \ \  C(\tilde x) & \text{ subject to } &  \tilde x \in \mathbb{\tilde X}
\eq
Since \eqref{eq:bfm} is quadratic, $\mathbb{X}$ is generally a nonconvex set.
OPF is thus a nonconvex problem and NP-hard to solve in general. 

\vspace{0.1in}
\begin{remark}
\textbf{Equivalence.}
By Theorem \ref{thm:bim=bfm} there is a bijection between $\mathbb V$ and
$\mathbb{\tilde X}$ and therefore OPF in the bus injection model and the branch
flow model are equivalent.   As we will see below some relaxations are easier to 
formulate in one model than the other.   We will also see in Part II of the paper that
some conditions for exact relaxation are easier to prove in one than the other model.
\end{remark}

\begin{remark}
\textbf{OPF variants.}
OPF as defined in \eqref{eq:OPFbim} and \eqref{eq:OPFbfm}  is a simplified version 
that ignores other important constraints such as line limits,  security constraints,
stability constraints, and chance constraints; see extensive surveys in \cite{Powerbk, Huneault91,Momoh99a,Momoh99b,Pandya08, Frank2012a, Frank2012b,
OPF-FERC-1, OPF-FERC-2, OPF-FERC-3, OPF-FERC-4, OPF-FERC-5, GanThomas2000}.
The  model presented here also ignores shunt elements.
Some of these (e.g. shunt elements and line limits) can be incorporated without any 
change to the results in this paper.  
\end{remark}

\begin{comment}
\slow{Stability constrained OPF - check Hsiao-Dong Chiang's website.
check "Practical OPF" 2009.}
\end{comment}



\subsubsection{OPF as QCQP}

Before we describe convex relaxations of OPF  we first show that,
when $C(V) := V^H C V$ is quadratic in $V$, OPF 
is indeed a quadratically constrained quadratic program (QCQP)
by converting it into the standard form.  
We will use the derivation in \cite{Bose-2012-QCQPt} for OPF \eqref{eq:OPFbim}
in bus injection model.   OPF \eqref{eq:OPFbfm} can similarly be converted into
a standard form QCQP.

To write \eqref{eq:OPFbim} in the standard form % \eqref{eq:defqcqp.1}, 
define the $(n+1) \times (n+1)$ admittance matrix $Y$ as
\bqn
Y_{ij} & = & \begin{cases}
\displaystyle
\sum_{k: k \sim i} y_{ik}, & \text{ if } i=j,\\
- y_{ij}, & \text{ if } i \neq j \text { and $i \sim j$}, \\
0 & \text{ otherwise}.\end{cases}
\eqn
$Y$ is symmetric but not necessarily Hermitian.   
Then
\bqn
s_j & := & V_j I_j^H \ = \ (e_j^H V) (I^H e_j)
\eqn
where $e_j$ is the $n$-dimensional vector with 1 in the $j$th entry
and 0 elsewhere.  Hence, since $I = YV$, we have
\bqn
s_j \ = \ \text{tr } \left( e_j^H VV^H Y^H e_j \right) 
	& = & \text{tr } \left( Y^H e_j e_j^H \right) VV^H
\\
	& = & V^H Y_j^H V
\eqn
where $Y_j^H := Y^H e_j e_j^H$.   $Y_j$ is an $n\times n$ matrix with its $j$th row
equal to the $j$th row of the admittance matrix $Y$ and all other rows equal
to the zero vector.   $Y_j^H$ is  in general not Hermitian so that 
$V^H Y_j^H V$ is in general a complex number.
Its real and imaginary parts can be expressed in terms of the Hermitian and
skew Hermitian components of $Y_j^H$ defined as:
\bq
\!\!\!\!\!
\Phi_j := \frac{1}{2} \left( Y_j^H + Y_j \right) &\!\!\!\!\!  \text{and} \!\!\!\!\! & 
\Psi_j := \frac{1}{2\ii} \left( Y_j^H - Y_j \right)
\label{eq:defPhiPsi}
\eq
Then 
\bqn
\text{Re}\,\, s_j = V^H \Phi_j V  & \text{and} & 
\text{Im}\, \, s_j = V^H \Psi_j V
\eqn
Let their upper and lower bounds be denoted by
\bqn
\underline{p}_j := \text{Re}\,\, \underline{s}_j & \text{and} & 
\overline{p}_j := \text{Re}\,\, \overline{s}_j
\\
\underline{q}_j := \text{Re}\,\, \underline{s}_j & \text{and} & 
\overline{q}_j := \text{Re}\,\, \overline{s}_j
\eqn



Let $J_j := e_j e_j^H$ denote the Hermitian matrix with a single 1 in
the $(j,j)$th entry and 0 everywhere else.
Suppose $C(V) := V^H C V$ for some Hermitian matrix $C$.
Then OPF \eqref{eq:OPFbim} can be written as a standard form QCQP:
\begin{subequations}
\bq
\!\!\!\!\!\!    \!\!\!\!\!\!\!
\min_{x\in \mathbb C^n} & \!\!\!\! & \!\!\!\!  V^H C V
\label{eq:bimOPF.b1}
\\
\!\!\!\!\!\!       \!\!\!\!\!\!\!
\text{s.t.}  & \!\!\!\! & \!\!\!\!
 	V^H \Phi_j V \leq \overline{p}_j, \  	V^H (-\Phi_j) V \leq -\underline{p}_j
\label{eq:bimOPF.b2}
\\
\!\!\!\!\!\!       \!\!\!\!\!\!\!   & \!\!\!\!  & \!\!\!\!
 		V^H \Psi_j V \leq \overline{q}_j, \ V^H (-\Psi_j) V \leq -\underline{q}_j
\label{eq:bimOPF.b3}
\\
\!\!\!\!\!\!       \!\!\!\!\!\!\!   & \!\!\!\!  & \!\!\!\!
		V^H J_j V \leq -\overline{v}_j, \ V^H (- J_j) V \leq -\underline{v}_j
\label{eq:bimOPF.b5}
\eq
\label{eq:OPFbim.2}
\end{subequations}
where $j\in N$ in \eqref{eq:OPFbim.2}.



\subsection{Feasible sets and relaxations: BIM}

The cost function of OPF is usually assumed to be convex.  The difficulty of OPF 
 thus arises mainly from the nonconvex feasible sets $\mathbb V$ (for bus injection model)
and $\mathbb{\tilde X}$ (for branch flow model).
The basic approach to deriving convex relaxations of OPF is to design convex
supersets of $\mathbb V$ (or $\mathbb{\tilde X}$) and minimize the same cost
functions over these convex supersets.  Different choices of convex supersets
lead to different relaxations, but these relaxations all provide a lower bound to OPF.
If an optimal solution of a convex relaxation happen to be in $\mathbb V$
(or $\mathbb{\tilde X}$) then it is also feasible and hence optimal for the original
OPF.

In the rest of this section  we  characterize the feasible sets of OPF.  The characterizations
 suggest several convex relaxations and we prove equivalence relations
among these relaxations.   In Part II of the paper we discuss sufficient conditions
that guaranteed exact relaxation.

\vspace{0.1in}
We now summarize the main results in  
\cite{Bose-2012-BFMe-Allerton, Bose-2013-BFMe} that characterize the feasible 
set $\mathbb V$ of OPF in \eqref{eq:OPFbim} in terms of partial matrices.  These
characterizations lead naturally to  SDP, chordal, and SOCP relaxations of OPF.

Given a voltage vector $V\in \mathbb V$ we can define a partial matrix $W_G$ by
(see e.g. \cite{Grone1984, Fukuda99exploitingsparsity, Nakata2003} for concepts
of partial matrices and \cite{Bose-2012-BFMe-Allerton, Bose-2013-BFMe} for their
application to OPF):
\begin{align*}
[W_G]_{jj} & := |V_j|^2
\\
[W_G]_{jk}  & := V_j V_k^H  \ =: \ [W_G]_{kj}^H
\end{align*}
Then the constraints
\eqref{eq:bimopf.1} and \eqref{eq:opfv}  imply that the partial matrix $W_G$ satisfies
 \footnote{The constraint
\eqref{eq:opfW.1} can also be written compactly in terms of the admittance matrix 
$Y$ as in \cite{Zhang2013}:
\bqn
\underline{s} \ \leq \  \text{diag } \left( WY^H \right) \ \leq \ \overline{s}
\eqn
}
\begin{subequations}
\bq
\underline{s}_j  \leq\!\!  \sum_{k: (j,k)\in E}\!\! y_{jk}^H\, \left( [W_G]_{jj} - [W_G]_{jk} \right) 
 \leq  \ \overline{s}_j,  j \in N
\label{eq:opfW.1}
\\
\underline{v}_j \leq [W_G]_{jj} \leq \overline{v}_j,  \qquad\qquad j \in N
\label{eq:opfW.2}
\eq
\label{eq:opfW}
\end{subequations}
As shown above these  constraints can also be written
in a (partial) matrix form as:
\bqn
\underline{p}_j & \leq\  \text{tr}\ \Phi_j W_G \ \leq & \overline{p}_j
\\
\underline{q}_j & \leq\  \text{tr}\ \Psi_j W_G \ \leq & \overline{q}_j
\\
\underline{v}_j & \leq\  \text{tr}\ J_j W_G \ \leq & \overline{v}_j
\eqn


The converse is not always true: given a partial matrix $W_G$ that satisfies \eqref{eq:opfW}
it is not always possible to recover a voltage vector $V$ in $\mathbb V$.
It is clear that {\em any} completion $W$ of such a $W_G$ would also satisfy
\eqref{eq:opfW} since $y_{jk}=0$ if $(j,k)\not\in E$.   We can recover a
voltage vector $V\in \mathbb V$ if $W$ happens to be psd rank-1
 because in that case it can be uniquely decomposed into 
$W= VV^H$ with $V\in \mathbb V$.  


We hence seek additional conditions on the partial matrix $W_G$ that guarantee  that
it has a psd rank-1 completion $W$ from which $V\in \mathbb V$ can be recovered.
To this end
we say that a partial matrix $W_G$ satisfies the {\em cycle condition} if, for every 
cycle $c$ in $G$,
\bq
\sum_{(i,j)\in c}\ \angle W_{ij} & = & 0   \mod 2\pi
\label{eq:cyclecond.2}
\eq

We recall 
that a partial matrix $W_F$ is defined to
be psd (or rank-1) if $W_F(q) \geq 0$ (or rank $W_F(q) = 1$) for all its 
principal submatrices $W_F(q)$ defined on all the maximal cliques $q$ of $F$.


The following result characterizes when a definite matrix $W$ is of rank 1 in terms of
its restriction onto $G$ or any chordal extension $c(G)$, i.e., in terms of its 
submatrices $W_G$ and $W_{c(G)}$.
It is proved in \cite[Theorem 3]{Bose-2012-BFMe-Allerton}, \cite{Bose-2013-BFMe}.
It implies that a partial matrix $W_G$ has a psd rank-1 completion $W$ if and only if
$W_G$ is $2\times 2$ rank-1 on $G$ and satisfies the cycle condition \eqref{eq:cyclecond.2}
if and only if it has a chordal extension $W_{c(G)}$ that is psd rank-1.
It leads to three convex relaxations of OPF -- SDP, chordal, and SOCP
relaxations, as explained below.
\begin{theorem}
\label{thm:rank1}
Fix a graph $G$ on $n$ nodes and any chordal extension $c(G)$ of $G$.
Given an $n\times n$ positive or negative 
semidefinite matrix $W$ the following are equivalent:
\bee 
 \item[(1) ] rank $W = 1$.
 \item[(2) ]  rank $W_{c(G)} = 1$.
  \item[(3) ]  rank $W_G(i,j) = 1$ for all $(i,j)\in E$ and  the partial matrix $W_G$ satisfies the cycle
 	 condition \eqref{eq:cyclecond.2}.
 \eee
\end{theorem}
\begin{comment}
\slow{Fix: avoid $V_i= V_j=0$, zero principle submatrix of rank-1 $W$.}
\end{comment}

\begin{remark}
\label{remark2}
As shown in \cite{Bose-2012-BFMe-Allerton}  the set of completions of a partial 
matrix $W_G$ that satisfies the condition in Theorem \ref{thm:rank1}(3) can 
consist of a  {single} positive semidefinite rank-1 matrix, or a {single}
 negative semidefinite rank-1 matrix, and  infinitely many indefinite
non-rank-1 matrices.
For OPF we are interested only in a partial matrix $W_G$ that is $2\times 2$ psd
($W(i,j)\succeq 0$ for all $(i,j)\in E$), in addition to the condition in
Theorem \ref{thm:rank1}(3).    Such a partial matrix $W_G$ cannot have a
negative definite completion.   Hence it must have a \emph{unique}
psd rank-1 completion $W$ (as well as indefinite non-rank-1 completions);
see \cite[Theorems 5 and 8]{Bose-2012-BFMe-Allerton}
and discussions therein.   We will construct this $W$ explicitly below.
\end{remark}

\begin{comment}
\slow{Check \cite{Sojoudi2012PES} for citation of Theorem \ref{thm:rank1}(3)?}
\end{comment}

The rank-1 condition is a property of the whole matrix $W$.    
Theorem \ref{thm:rank1} characterizes this in terms of two different submatrices
$W_G$ and $W_{c(G)}$ of $W$, defined on graph $G$ and its chordal 
extension $c(G)$ respectively.
This is important because the submatrices are typically much smaller than $W$ and
can be much more efficiently computed for large sparse networks.
The theorem thus allows us to solve simpler problems in terms of partial matrices, 
as we now explain.

\slow{SHould be $(n+1)\times (n+1)$ matrices and $\mathbb S^{n+1}$ ?}
\slow{Change $\mathbb W_1$ to $\mathbb W$ and $\mathbb W_2$ to $\mathbb W_G$?
We did use $\mathbb W$ once generically to refer to $\mathbb W_1, \mathbb W_{c(G)}, \mathbb  W_2$.}

Define the set of $n\times n$ Hermitian matrices:
\begin{equation}
\begin{array}{rl}
 \mathbb W_1 \ := \  \{W \in \mathbb S^{n} \ \vert \ & \!\!\!\!\! W_G \text{ satisfies } 
		\eqref{eq:opfW}, 
\nonumber 
\\
   		&\!\!\!\!\!  W\succeq 0, \text{ rank } W = 1 \}
\end{array}
\label{eq:defW1}
\end{equation}
Fix any chordal extension $c(G)$ of $G$ and define the set of Hermitian \emph{partial}
matrices $W_{c(G)}$:
\begin{equation}
\begin{array}{rl}
 \mathbb W_{c(G)} \ := \ \{W_{c(G)}  \ \vert \ & \!\!\!\!\! W_G \text{ satisfies } \eqref{eq:opfW}, 
\nonumber 
\\
    	 &  \!\!\!\!\! W_{c(G)} \succeq 0, \text{ rank } W_{c(G)} = 1 \}
\end{array}
\label{eq:defWcG}
\end{equation}
where given a $W_{c(G)}$, $W_G$ denotes the submatrix of $W_{c(G)}$ 
with off diagonal entries $[W_G]_{jk}$ defined only for $(j,k)\in E$.
Finally define the set of Hermitian partial matrices $W_G$:
\begin{equation}
\begin{array}{rl}
 \mathbb W_2 \ := \ \{W_{G}  \ \vert & \!\!\!\!\! W_G \text{ satisfies } \eqref{eq:opfW}, 
 			\eqref{eq:cyclecond.2}, W_G(i,j) \succeq 0, 
\nonumber 
\\
    	 &  \!\!\!\!\!\!\!\! \text{ rank } W_G(i,j) = 1 \text{ for all } (i,j)\in E \}
\end{array}
\label{eq:defW2}
\end{equation}
Remark \ref{remark2} immediately implies
\begin{corollary}
\label{coro:eq}
Given a partial matrix $W_{c(G)} \in \mathbb W_{c(G)}$ or $W_G \in \mathbb W_2$
there is a unique psd rank-1 completion $W \in \mathbb W_1$.
\end{corollary}

Recall that two sets $A$ and $B$ are \emph{equivalent}, denoted by $A\equiv B$,
if there is a bijection between them.  
Even though $\mathbb W_1, \mathbb W_{c(G)}, \mathbb W_2$ are different
(e.g. their matrices have different dimensions) Theorem \ref{thm:rank1} and Corollary
\ref{coro:eq} imply that they are all equivalent to the feasible set of OPF.
\begin{corollary}
\label{coro: FS}
$\mathbb V \equiv \mathbb W_1 \equiv \mathbb W_{c(G)} \equiv \mathbb W_2$.
\end{corollary}

Corollary \ref{coro: FS} suggests three equivalent problems to OPF.
We assume the cost function $C(V)$ in OPF depends on $V$ only through the
$G$-partial matrix $W_G$.   For example if the cost is total real line loss in the 
network then $C(V) = \sum_j \text{Re } s_j = \sum_j \sum_{k:(j,k)\in E} 
\text{Re} \left([W_G]_{jj} - [W_G]_{jk} \right) y_{jk}^H$.  If the
cost is a weighted sum of real generation power then
$C(V) = \sum_j \left(c_j \, \text{Re } s_j + p_j^{d} \right)$ where $p_j^{d}$ are the given real power
demands at buses $j$; again $C(V)$ is a function of the $G$-partial matrix $W_G$.
Then OPF \eqref{eq:OPFbim} is equivalent to 
\bq
\underset{W}{\text{min}}   \ C(W_G) \ & \text{subject to} &   W \in \mathbb W
\label{eq:bimeqp}
\eq
where $\mathbb W$ is any one of the sets $\mathbb W_1, \mathbb W_{c(G)}, \mathbb W_2$
and the variable  $W$ is of appropriate dimension.   This makes use of the fact that these
four problems have the same objective function and there is a bijection 
among their feasible sets.
More specifically, 
given an optimal solution $W^*$ in $\mathbb W_1$, since $W$ is rank-1, it can be uniquely
decomposed into $W^* = V^*(V^*)^H$.  Then $V^*$ is in $\mathbb V$ and an optimal
solution of OPF \eqref{eq:OPFbim}.   Alternatively given an optimal solution $W_F^*$ in
$\mathbb W_{c(G)}$ or $\mathbb W_2$, Corollary \ref{coro:eq} guarantees that 
$W_F^*$ has a psd rank-1 completion $W^*$ in $\mathbb W_1$ from which an optimal 
$V^*\in \mathbb V$ can be recovered through spectral decomposition.
For a partial matrix $W_G^* \in \mathbb W_2$ or $W_{c(G)}^* \in \mathbb W_{c(G)}$
there is an alternative, a much more direct, construction of $V^*\in \mathbb V$
(see \cite{Bose-2012-BFMe-Allerton} and the distributed angle recovery algorithm
in \cite{Farivar-2013-BFM-TPS1}).

\begin{comment}
\slow{Remove for TCNS submission.  Clean up for lecture notes: 
For OPF-socp if the optimal solution $W_G$ is $2\times 2$ rank-1 on $G$
and satisfies the cycle condition \eqref{eq:cyclecond.2} (a radial network automatically
satisfies \eqref{eq:cyclecond.2}) then a unique $V^*$ 
can be  constructed explicitly as follows.  
Let $T$ be an arbitrary spanning tree of ${G}$.   Let $\mathbb P_{ij}$
denote the unique path from node $i$ to node $j$ in $T$.
For $i = 1, \dots, n$, let 
\bq
|V_i^*|  & := &  \sqrt{\left[ W_G \right]_{ii}}  
\label{eq:V.1}
\\
\angle V_i^* & := &   \sum_{(j,k)\in \mathbb P_{1i}} \angle \left[ W_G \right]_{jk}
\label{eq:V.2}
\eq
Without loss of generality set $\angle V_1 = 0$ in this construction
(otherwise, add $\angle V_1$ to \eqref{eq:V.2}).  
Then it can be checked that $V^*$ is an optimal solution of OPF \eqref{eq:bimOPF}.
}
\end{comment}

Hence solving OPF \eqref{eq:OPFbim} is equivalent to solving \eqref{eq:bimeqp}
over any of $\mathbb W_1, \mathbb W_{c(G)}, \mathbb W_2$ with appropriate
matrix variables.
The difficulty with solving \eqref{eq:bimeqp} is that the feasible sets 
$\mathbb W_1$, $\mathbb W_{c(G)}$, and $\mathbb W_2$ are still
nonconvex due to the rank-1 constraints and the cycle condition \eqref{eq:cyclecond.2}.   
Their removal leads to the SDP, chordal, and SOCP relaxations of OPF
respectively.

Relax $\mathbb W_1$ to a convex subset of $\mathbb S^n$:
\begin{equation}
\begin{array}{rl}
 \mathbb W_1^+ \ := \  \{W \in \mathbb S^n  \ \vert \ & \!\!\!\!\! W_G \text{ satisfies } 
		\eqref{eq:opfW},   W\succeq 0 \}
\end{array}
\label{eq:defW1+}
\end{equation}
Relax $\mathbb W_{c(G)}$ to a convex set of Hermitian partial matrices:
\begin{equation}
\begin{array}{rl}
 \mathbb W_{c(G)}^+ \ := \ \{W_{c(G)}  \ \vert \ & \!\!\!\!\! W_G \text{ satisfies } \eqref{eq:opfW}, 
			 W_{c(G)} \succeq 0 \}
\end{array}
\label{eq:defWcG+}
\end{equation}
Relax $\mathbb W_G$ to a convex set of Hermitian partial matrices
by dropping both the $2\times 2$ rank-1 condition and the cycle condition:
\begin{equation}
\begin{array}{rl}
 \mathbb W_2^+ \ := \ \{W_{G}  \ \vert \ & \!\!\!\!\! W_G \text{ satisfies } \eqref{eq:opfW}, 
 			
\nonumber 
\\
    	 &  \!\!\!\!\! W_G(j,k) \succeq 0,   \ (j,k)\in E \}
\end{array}
\label{eq:defW2+}
\end{equation}
Define the problems:
\\
\noindent
\textbf{OPF-sdp:}
\bq
\label{eq:bimOPF-sdp}
% \!\!\!\!\!\!\!\!\!\!\!\!\! 
\hspace{-0.315in}
\underset{W}{\text{min}}   \ C(W_G) \ & \text{subject to} &   W \in \mathbb W_1^+
\eq
\noindent
\textbf{OPF-ch:}
\bq
\label{eq:bimOPF-ch}
\underset{W_{c(G)}}{\text{min}}   \ C(W_G) \ & \text{subject to} &   W_{c(G)} \in \mathbb W_{c(G)}^+
\eq
\noindent
\textbf{OPF-socp:}
\bq
\label{eq:bimOPF-socp}
\hspace{-0.285in}
\underset{W_G}{\text{min}}   \ C(W_G) \ & \text{subject to} &   W_G \in \mathbb W_2^+
\eq
Since $\mathbb W_1 \subseteq \mathbb W_1^+$, 
$\mathbb W_{c(G)} \subseteq \mathbb W_{c(G)}^+$, 
$\mathbb W_2 \subseteq \mathbb W_2^+$, OPF-sdp, OPF-ch, OPF-socp provide
lower bounds on the optimal value of OPF \eqref{eq:OPFbim} in light of
Corollary \ref{coro: FS}.

We make two comments on these semidefinite programs.  First
the condition $W_G(j,k)\succeq 0$ in the definition of $\mathbb W_2^+$ is 
equivalent to
\bqn
[W_G]{jj} \geq 0, \ [W_G]_{kk} \geq 0, \  [W_G]_{jj}[W_G]_{kk} \geq \left| [W_G]_{jk} \right|^2
\eqn
This is a second-order cone and
hence OPF-socp is indeed an SOCP in the rotated form.  % \eqref{eq:defsocp.b}.
Second OPF-ch is  a convex chordal relaxation in the standard form.  % \eqref{eq:defcr}.
SOCP relaxation for OPF seems to be first observed in \cite{Sojoudi2012PES} for
the bus injection model and in \cite{Farivar2011-VAR-SGC} for the branch flow model.
%  discussed in Section \ref{sec:bfm}).
Chordal relaxation for OPF is first proposed in \cite{Jabr2012}.

For a mapping $f: A\rightarrow B$ let $f(A)$ denote the set 
$\{f(x)\ | \ x\in A\} \subseteq B$.   For two sets $A$ and $B$ that are
not necessarily in the same space we say that $A$ is an \emph{equivalent
subset} of $B$, denoted by $A\sqsubseteq B$, if there is a mapping 
$f : A \rightarrow B$ such that $f(A) \subseteq B$ and $f$ is a bijection 
from $A$ to $f(A)$.
Clearly $A\equiv B$ if and only if $A\sqsubseteq B$ and $B \sqsubseteq A$.
The feasible set of OPF \eqref{eq:OPFbim} is an equivalent subset of the feasible
sets of the relaxations, as the following results from \cite{Bose-2012-BFMe-Allerton,
Bose-2013-BFMe} show.
\begin{theorem} [\cite{Bose-2012-BFMe-Allerton, Bose-2013-BFMe}]
\label{thm: bimR}
\bee
\item If $G$ is radial then 
	$\mathbb V \sqsubseteq \mathbb W_1^+ \equiv \mathbb W_{c(G)}^+ \equiv \mathbb W_2^+$.
\item If $G$ has cycles then
	$\mathbb V \sqsubseteq \mathbb W_1^+ \equiv \mathbb W_{c(G)}^+ \sqsubseteq \mathbb W_2^+$.
\eee
\end{theorem}


Let $C^*, C_{sdp}, C_{ch}, C_{socp}$ be the optimal values of OPF,
OPF-sdp, OPF-ch, OPF-socp respectively.   
Theorem \ref{thm: bimR} and Corollary \ref{coro: FS} directly imply
\begin{corollary}
\label{coro:bimR}
\bee
\item If $G$ is radial then $C^* \geq C_{sdp} = C_{ch} = C_{socp}$.
\item If $G$ has cycles then $C^* \geq C_{sdp} = C_{ch} \geq C_{socp}$.
\eee
\end{corollary}




\subsection{Feasible sets and relaxations: BFM}
\label{subsec:Relabfm}

The DistFlow equations \eqref{eq:df.a}  for radial networks can be extended
for mesh networks:
\begin{subequations}
\bq
\sum_{k: j\rightarrow k} S_{jk} & = & \sum_{i: i\rightarrow j} \left( S_{ij} - z_{ij} \ell_{ij} \right)
		 + s_j, \quad j \in N^+
\label{eq:mdf.1}
\\
v_j - v_k & = & 2\, \text{Re} \left(z_{jk}^H S_{jk} \right) - |z_{jk}|^2 \ell_{jk}, \ \ j\rightarrow k \in \tilde E
\nonumber
\\
\label{eq:mdf.2}
\\
\ell_{jk} v_j & = & |S_{jk}|^2, \quad j\rightarrow k \in \tilde E
\label{eq:mdf.3}
\eq
\label{eq:mdf}
\end{subequations}
Note that \eqref{eq:mdf.1} holds for $j=0$ for mesh network.
For radial networks \eqref{eq:df.1} only holds for $j\neq 0$ and the case
of $j=0$ becomes the boundary conditions \eqref{eq:df.4} that initiates
the recursion.
Let the set of solutions $x := (S, \ell, v, s_0, s)$ be:
\bqn
{\mathbb X}_{m} & := & \{ x \in \mathbb R^{3m+3n+2} \ \vert \ x \text{ satisfies } 
		\eqref{eq:mdf},  \eqref{eq:opfv}, \eqref{eq:opfs}  \}
\eqn
$\mathbb X_m$ is a relaxation of $\mathbb{\tilde X}$ in the sense that
$\mathbb{\tilde X} \sqsubseteq \mathbb X_m$ defined by the mapping
$h$ defined in Section \ref{subsec:bfmr} (that $h$ is a bijection between
$\mathbb{\tilde X}$ and $h(\mathbb{\tilde X})$ is proved below).

The set $\mathbb X_m$ is still nonconvex because of the
 quadratic equalities in \eqref{eq:mdf.3}.  Relaxes them  to inequalities:
\bq
\ell_{jk} v_j & \geq &  |S_{jk}|^2,  \qquad   (j, k)\in \tilde{E}
\label{eq:mdf.socp}
\eq
Define the set: 
 \bq
{\mathbb X}^+ & := & \{ x \in \mathbb R^{3m+3n+2} \ \vert \ x \text{ satisfies } 
		\eqref{eq:mdf.1}, \eqref{eq:mdf.2}, \eqref{eq:mdf.socp}, 
\nonumber
\\
			& & \qquad\qquad\qquad\qquad\qquad \quad \ 
					    \eqref{eq:opfv}, \eqref{eq:opfs}  \}
\label{eq:defXm}
\eq
Clearly $\mathbb{\tilde X} \sqsubseteq \mathbb X_m \subseteq X^+$;
see Figure \ref{fig:Xsets}.

We now characterize the subset of $\mathbb X_m$ that is equivalent to 
$\mathbb{\tilde X}$.   This characterization also pinpoints where the model
\eqref{eq:mdf} fails for mesh network, leading to an exact relaxation result
for AC mesh networks using phase shifters explained in Part II of the paper.

Most of the discussion below involves a fixed $s$.  To simplify exposition
we will abuse notation and use $x$ to denote either $(S, \ell, v, s_0)$ or
$(S, \ell, v, s_0, s)$ with the given $s$, depending on the context, and use
$\mathbb X_m$ and $\mathbb X_m(s)$ interchangeably to denote 
$\mathbb X_m$ in \eqref{eq:defXm} or the projection of $\mathbb X_m$
to the fixed $s$.   The meaning should be clear from the context.

The mapping $h$ defined in Section \ref{subsubsec:re} 
relaxes a voltage $V_j$ or current $I_{jk}$ from a point in the complex
plane into a circle with its magnitude as the radius of the circle.  Fix any $s$.
While \eqref{eq:bfm} specifies $2m+n+1$ (nonlinear) equations in $2m+n+1$ complex
variables $(S, I, V, s_0)$, 	\eqref{eq:mdf} specifies $2(m+n+1)$ equations in 
$3m+n+2$ real variables $x := (S, \ell, v, s_0)$.
Since $m\geq n$ ($\tilde G$ is connected) there are generally insufficient number 
of equations to determine uniquely all the variables $x$ when $\tilde G$ contains cycles.
When $\tilde G$ is a tree,
then $m=n$ and both the number of equations and the number of real variables 
become  $4n+2$.
Indeed the results in \cite{Farivar-2013-BFM-TPS} shows that when $\tilde G$ is a
tree, $h: \mathbb{\tilde X}(s) \rightarrow \mathbb X_m(s)$ is bijective 
and any $x\in \mathbb X_m(s)$
can be mapped to a power flow solution $\tilde x \in \mathbb{\tilde X}(s)$.
Otherwise $h(\mathbb{\tilde X}(s)) \subsetneq \mathbb X_m(s)$, i.e., 
$h$ is not surjective on $\mathbb X_m(s)$ and there are $x$ that satisfy \eqref{eq:mdf} but
no phase angles can be assigned to $\sqrt{v_j}$ to obtain a power flow solution 
$\tilde x \in \mathbb{\tilde X}(s)$.
We now characterize the subset $h(\mathbb{\tilde X}(s))$ of $\mathbb X_m(s)$ over which 
$h$ is surjective and construct its inverse $h^{-1}$.

Given an $ x := (S, \ell, v, s_0) \in \mathbb R^{3m+n+2}$ 
define $\beta := \beta({x}) \in \mathbb R^m$ by
\bq
\beta_{jk}( x) & := & \angle \left( v_j - z_{jk}^H S_{jk} \right), \quad  j \rightarrow k\in \tilde E
\label{eq:defb.1}
\eq
Even though $x$ does not include phase angles of $V$ it turns out that $x$
``implies'' a phase angle difference across each line $(i,j)\in \tilde E$
given by $\beta_{ij}(x)$ \cite[Theorem 2]{Farivar-2013-BFM-TPS}.  
Whether an $x\in \mathbb X(s)$ can be mapped to a power flow solution 
$\tilde x \in \mathbb{\tilde X}(s)$ depends on whether there exist $\theta$ such
that $\theta_j - \theta_k = \beta_{jk}(x)$.
To state this precisely let $B$ be the $m\times n$ (transposed) reduced incidence 
matrix of $\tilde{G}$:
% obtained from $C$ defined in Section \ref{subsec:la}
% by removing its row corresponding to bus 0 and taking the transpose:
\bqn
B_{lj} & = & \begin{cases}
		1 & \text{ if edge $l \in \tilde E$ leaves node $j$} \\
		-1 & \text{ if edge $l \in \tilde E$ enters node $j$} \\
		0 & \text{ otherwise}
		\end{cases}
		\quad\quad  
% \label{eq:defB}
\eqn
%
Consider the set of $x$ such that 
\bq
\!\!\!\!\!\!
\exists \theta(x) \text{ that solves }\ 
	B\theta &\!\!\! = \!\!\! & \beta(x)  \mod 2\pi
\label{eq:cyclecond.1}
\eq
i.e., $\beta(x)$ is in the range space of $B$ (mod $2\pi$).
A solution $\theta(x)$, if exists, is unique in  $[-\pi, \pi)^n$.
To provide a more explicit characterization of those $x\in \mathbb X_m(s)$ 
that satisfy \eqref{eq:cyclecond.1}, fix any spanning tree $T = (N, E_T)$ of $\tilde G$.   
We can assume without loss of generality 
(possibly after re-labeling some of the links) that $E_T$ consists of links $l = 1, \dots, n$.  
Then $B$ can be partitioned into
\bq
B & = & \begin{bmatrix}
		B_T  \\ B_{\perp}
		\end{bmatrix}
\label{eq:B}
\eq
where the $n\times n$ submatrix $B_T$ corresponds to links in $T$ and the 
$(m-n) \times n$ submatrix $B_{\perp}$ corresponds to links in $T^\perp := G\setminus T$.
Similarly partition $\beta(x)$ into
\bq
\beta(x) & = & \begin{bmatrix}
		\beta_T (x) \\  \beta_{\perp} (x)
		\end{bmatrix}
\label{eq:defb.2}
\eq 
\begin{theorem}[\cite{Farivar-2013-BFM-TPS} Theorems 2 and 4]
\label{thm:anglecond}
An $x \in \mathbb X_m(s)$ satisfies \eqref{eq:cyclecond.1} if and only if
	\bq
	B_{\perp} B_T^{-1} \beta_T(x) & = & \beta_{\perp}(x)
	\quad\quad (\text{mod }2\pi)
	\label{eq:anglecond}
	\eq
	In that case $\theta(x) = \mathcal P \left(B_T^{-1}\beta_T(x) \right)$
	where $\mathcal P(\phi)$ projects $\phi$ to $[-\pi, \pi)^n$.
\end{theorem}
\vspace{0.1in}
Theorem \ref{thm:anglecond} determines when a given set of voltage magnitudes $v$ can be
assigned phase angles $\theta(x)$ so that the resulting complex voltages 
$V$ form a power flow solution.
When it holds, the angle recovery condition \eqref{eq:anglecond} has a familiar interpretation:
the voltage angle differences implied by $x$ sum to zero (mod $2\pi$) around any cycle
 \cite[Theorem 2(2)]{Farivar-2013-BFM-TPS}.

The subset of $\mathbb X_m(s)$ that satisfies \eqref{eq:cyclecond.1} are those 
that are equivalent to power flow solutions $\mathbb{\tilde X}(s)$.   For these $x$
an inverse $h^{-1}(S, \ell, v, s_0) = (S, I, V, s_0)$ can be defined in terms of $\theta(x)$
from $\mathbb{R}^{3m+n+2}$ to $\mathbb{C}^{2m+n+1}$ by (recall $\angle V_0 = 0^\circ$):
\begin{subequations}
\bq
V_j & := & \sqrt{v_j} \ e^{\ii \theta_j(x)},  \quad j \in N
% \label{eq:bfs.2}
\\
I_{jk} & := & \sqrt{\ell_{jk}}\ e^{\ii (\theta_j(x) - \angle S_{jk})}, \  (j,k) \in \tilde E
% \label{eq:bfs.3}
\eq
\label{eq:defhinv}
\end{subequations}
Define the set:
 \bqn
{\mathbb X}(s) & := & \mathbb X_m(s) \ \cap\ \{ x \in \mathbb R^{3m+n+2} \ \vert \ x \text{ satisfies } 
%		(\ref{eq:bfm.1a}), \eqref{eq:opfB.2}, \eqref{eq:Kirchhoff.2c}, \eqref{eq:Kirchhoff.2d},
		\eqref{eq:cyclecond.1}  \}
\eqn
The following result follows directly from \cite[Theorems 2, 4]{Farivar-2013-BFM-TPS}.
\begin{theorem} [\cite{Farivar-2013-BFM-TPS}]
\label{thm:bfm.1}
\bee
\item For general networks $\tilde G$, 
	$\mathbb{\tilde X}(s) \equiv \mathbb X(s) \subseteq \mathbb X_m(s) \subseteq \mathbb X^+(s)$.
\item For radial networks $\tilde G$, 
	$\mathbb{\tilde X}(s) \equiv \mathbb X(s) = \mathbb X_m(s) \subseteq \mathbb X^+(s)$.
\eee
\end{theorem}
The theorem is illustrated in Figure \ref{fig:Xsets} (including $s$ as a variable).
%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
\centering
\includegraphics[width=0.39\textwidth]{figures/fig-Xsets.pdf}
\caption{Feasible sets $\mathbb{\tilde X}$ of OPF in the branch flow model, its equivalent
	set $\mathbb X$ (defined by the mapping $h$)
	and its relaxations $\mathbb X_m$, $\mathbb X_m^+$.  If $\tilde G$ is radial then
	$\mathbb X = \mathbb X_m$.
}
\label{fig:Xsets}
\end{figure}
%%%%%%%%%%%%%%%%


The three sets $\mathbb X$, $\mathbb X_m$, $\mathbb X_m^+$
define the following three optimization problems.
We assume the cost function $c(\tilde x)$ in OPF \eqref{eq:OPFbfm} depends on
$\tilde x := (S, I, V, s_0, s) \in \mathbb C^{2m+2n+1}$ only through 
$x := h(\tilde x) = (S, \ell, v, v_0, s) \in \mathbb R^{3m+3n+2}$.
For example if the cost is total real line loss in the network then
$c(\tilde x) = \sum_{(j, k) \in \tilde{E}} \, \text{Re}\, z_{jk} \ell_{jk}$.
If the cost is a weighted sum of real generation power then
$c(\tilde x) = \sum_j (c_j p_j + p_j^{d})$ where $p_j$ are the real parts of
$s_j$ and $p_j^{d}$ are the given real power
demands at buses $j$; again $c(\tilde{x})$ depends only on $x$.
Consider:
\\
\noindent
\textbf{OPF:}
\begin{subequations}
\begin{align*}
& \underset{ x } {\text{min}}   \ \  c( x) \quad
 \text{ subject to } \quad  x \in \mathbb X
\end{align*}
\end{subequations}

\noindent
\textbf{OPF-nc:}
\begin{subequations}
\begin{align*}
& \underset{ x} {\text{min}}   \ \  c( x) \quad
\text{ subject to} \quad  x \in \mathbb X_m
\end{align*}
\end{subequations}

\noindent
\textbf{OPF-socp:}
\begin{subequations}
\begin{align*}
& \underset{ x } {\text{min}}   \ \  c( x) \quad
\text{ subject to } \quad  x \in \mathbb X_m^+
\end{align*}
\end{subequations}

Let $C^*$ be the optimal cost of OPF \eqref{eq:OPFbfm} in the branch flow model.
Let $C_{opf}$, $C_{nc}$, $C_{socp}$ be the optimal costs of OPF, OPF-nc, OPF-socp
respectively.
The following result follows directly from Theorem \ref{thm:bfm.1}.
\begin{corollary}
\label{coro:bfm.1}
\bee
\item[(1)] For general networks $\tilde G$,  $C^* = C_{opf} \geq C_{nc} \geq C_{socp}$.

\item[(2)] For radial networks $\tilde G$, $C^* = C_{opf} = C_{nc} \geq C_{socp}$.
\eee
\end{corollary}


\begin{comment}
\slow{Remove for TCNS submission FROM: 
========================================
}
We say OPF-socp is \emph{exact (with respect to OPF)} if every
optimal solution $x^*$ of OPF-socp attains equality in \eqref{eq:Kirchhoff.2e}
and satisfies \eqref{eq:cyclecond.2} so that an optimal solution to OPF can 
be recovered.  
An algorithm similar to that presented in the previous subsection on Solution
Strategy
Section \ref{subsec:ss} 
can be used 
 to compute an optimal OPF solution from $x^*$.   Algebraically,
for any optimal solution $x^*$ of OPF-socp that attains equality in 
\eqref{eq:Kirchhoff.2e} and satisfies \eqref{eq:cyclecond.2}, there is a unique 
$\theta(x^*)$ in $ [-\pi, \pi)^n$.
The inverse $\tilde x := h^{-1}(x^*)$ is an optimal point for OPF.

We now turn to sufficient conditions under which OPF-socp is exact.
We present the results first for AC radial networks and then for DC mesh
networks.  Finally we show that the case of AC mesh networks can be
reduced to the case of AC radial networks using phase shifters.




\slow{Move this to the next subsection?}
We now comment on the computational aspect of these three relaxations.
First the choice of the chordal extension $c(G)$ of $G$ determines the number
of variables in OPF-ch and hence the required computation effort, but
it does not affect its optimal value.
As discussed in earlier, a good choice of  
A good choice of $c(G)$ is nontrivial.   In the worst case OPF-ch can require as much effort as
OPF-sdp,  but simulation results on IEEE test systems
in \cite{Bose-2013-BFMe} confirm that it can be much more efficiently solved than
OPF-sdp when the network is large and sparse, as practical systems are.
Indeed the numbers of lines in IEEE test systems (with 14, 30, 57, 118, 300
buses) are less than 1.6 times the numbers of buses, much less than the squares
of them.

Second though all OPF-sdp, OPF-ch, and OPF-socp are convex and hence
can be solved in polynomial time, SOCP in general requires a much smaller 
computational effort than SDP for large sparse networks.
Indeed $G$ is a subgraph of any chordal
extension $c(G)$  which is a subgraph of the complete graph defined
on $N$, and hence the number of complex variables (matrix entries) is 
 the smallest in OPF-socp $(|W_G|)$, the largest in OPF-sdp $(n^2)$, 
 with OPF-ch typically in between.

Finally, and  most importantly, Corollary \ref{coro:bimR}
suggests that, when $G$ is a tree, we should \emph{always} solve OPF-socp.
When $G$ has cycles then there is a tradeoff between computational effort and
exactness in deciding between solving OPF-socp or OPF-sdp/OPF-ch.
Between OPF-sdp and OPF-ch, OPF-ch seems much more preferable
as they have the same accuracy (in terms of exactness) but OPF-ch is
much faster to solve for large sparse networks, as discussed above.

\slow{Remove for TCNS submission TILL: 
======================================
}
\end{comment}



\subsection{Equivalence}
\label{sec:eq}


Corollary \ref{coro: FS} establishes a bijection between  $\mathbb W_2$ and
the feasible set $\mathbb V$ of OPF in the bus injection model.
Theorem \ref{thm:bfm.1} establishes a bijection between $\mathbb X$ and
the feasible set $\mathbb{\tilde X}$ of OPF in the branch flow model. 
Theorem \ref{thm:bim=bfm} hence implies that there is a bijection between the
feasible sets $\mathbb V$ and $\mathbb X$ of OPF in the bus injection model 
and the branch flow model respectively.
Moreover the SOCP relaxations are equivalent in these two models.
It is in this sense that the models are equivalent.
\begin{theorem} [\cite{Bose-2012-BFMe-Allerton, Bose-2013-BFMe}]
\label{thm:eq}
$\mathbb W_2 \equiv \mathbb X$ and 
$\mathbb W_2^+ \equiv \mathbb X^+$.
\end{theorem}

The bijection between $\mathbb W_2^+$ and $\mathbb X^+$ used to prove the
second assertion defined as follows.
Let $\mathbb W_G \subseteq \mathbb C^{2m+n+1}$ denote the set of hermitian 
$G$-partial matrices.   Let ${x} := (S, \ell, v_0, v)$ denote vectors in $\mathbb R^{3m+n+1}$.
Define the mapping $g :\mathbb W_G \rightarrow \mathbb R^{3m+n+1}$ by 
${x}  = g(W)$ where 
\bqn
v_j & := &  [W_G]_{jj} \quad \text{for }  j\in N^+
\label{eq:g.1}
\\
S_{jk} &:= &   y_{jk}^H \left( [W_G]_{jj} - [W_G]_{jk} \right)  % \ \text{for }  j\rightarrow k 
\label{eq:g.2}
\\
\ell_{jk} & \!\!\!   := \!\!\!   &   |y_{jk}|^2 \left( [W_G]_{jj} + [W_G]_{kk} - [W_G]_{jk} - [W_G]_{kj} \right)
% \  \text{for } j \rightarrow k
\label{eq:g.3}
\eqn
Its inverse $g^{-1}: \mathbb R^{3m+n+1} \rightarrow \mathbb W_G$ is 
$W_G = g^{-1}(x)$ where
$[W_G]_{jj} := v_j$  for $j \in N^+$ and $[W_G]_{jk} := v_j - z_{jk}^H S_{jk} =: [W_G]_{kj}^H$
for $j\rightarrow k$.

% \bqn
% [W_G]_{jj} & :=  & v_j \quad \text{for } j\in N^+
% \label{eq:ginv.1} 
% \\
% [W_G]_{jk} & :=  &  v_j - z_{jk}^H S_{jk}  \ =: \ [W_G]_{kj}^H \quad \text{for } j \to k
% \label{eq:ginv.2}
% \eqn

%
\begin{comment}
\slow{Remove for TCNS submission.}
The next result implies that $g$ and $g^{-1}$ restricted to $\mathbb W_2^+$ $(\mathbb W_2)$
and $\mathbb X_2^+$ $(\mathbb X_2)$ respectively are indeed inverse of each other.

Second define the set of $G$-partial matrices that are in $\mathbb W_2^+$
but do not satisfy the cycle condition \eqref{eq:cyclecond}:
\begin{align*}
\FF_2^{nc} &:= \left\{ W_G \ \vert \  W_G=W_G^\herm, W_G \text{ satisfies }
	\eqref{eq:opfW.1}-\eqref{eq:opfW.2}, 
W_G(e) \succeq 0, \rank {W_G}(e) = 1 \text{ for  $e \in E$} \right\}
\end{align*}
Clearly $\mathbb W_2 \subseteq \mathbb W_2^{nc} \subseteq W_2^+$.
Then the same argument as in Theorem \ref{thm:branch} implies that $g$ and 
$g^{-1}$ define a bijection between $\mathbb W_2^{nc}$ and $\mathbb X_2^{nc}$.

\slow{Distributed algorithms based on BFM in \cite{Li-2013-PhD}.
Use of BFM for DR in Lina's paper.}
\end{comment}




\section{Conclusion}
\label{sec:c}

We have presented the bus injection model and branch flow model, 
formulated several convex relaxations of optimal power flow, and proved
their equivalence.   These results suggest a new approach to
solving OPF described in Figure \ref{fig:SolStrat}.
%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
\centering
\includegraphics[width=0.49\textwidth]{figures/fig-SolStrat.pdf}
\caption{Solving OPF based on convex relaxations.
}
\label{fig:SolStrat}
\end{figure}
%%%%%%%%%%%%%%%%

The key for this solution strategy is that the convex relaxations are exact
so that an optimal solution of the original OPF problem can be recovered.  
In Part II of this paper we summarize sufficient conditions that guarantee
exact relaxation.



